Safety Verification of Declarative Smart Contracts

Smart contracts manage a large number of digital assets nowadays. Bugs in these contracts have led to significant financial loss. Verifying the correctness of smart contracts is, therefore, an important task. This paper presents an automated safety verification tool, DCV, that targets declarative smart contracts written in DeCon, a logic-based domain-specific language for smart contract implementation and specification. DCV proves safety properties by mathematical induction and can automatically infer inductive invariants using heuristic patterns, without annotations from the developer. Our evaluation on 20 benchmark contracts shows that DCV is effective in verifying smart contracts adapted from public repositories, and can verify contracts not supported by other tools. Furthermore, DCV significantly outperforms baseline tools in verification time.

==> sec_inference-rules-bak.tex <==
The procedure EncodeRuleBody is defined by two sets of inference rules.
The first judgment of the form
$\Gamma, \tau \vdash r \hookrightarrow \phi$ 
states that a DeCon rule $r$ is encoded by a boolean formula $\phi$
under context $\Gamma$ and $\tau$.
The second judgment of the form
$ \Gamma,\tau \vdash \var{Pred} \rightsquigarrow \phi $
states that a predicate $\var{Pred}$ is encoded by
a formula $\phi$ under context $\Gamma$ and $\tau$.
The contexts ($\Gamma$ and $\tau$) of both judgement forms
are defined the same as the input of Algorithm~\ref{alg:transform-rule}.

%The syntax of a DeCon rule $r$ and a predicate $\var{Pred}$
%is defined in Section~\ref{sec:language}.

The judgment $\Gamma, \tau \vdash r \hookrightarrow \phi$
is defined by the following inference rules:
\[
\infer[(Join1)]{
    \Gamma,\tau \vdash H(\bar{y}) \dldeduce R(\bar{x}) \hookrightarrow \phi
}{
    \Gamma,\tau \vdash R(\bar{x}) \rightsquigarrow \phi
}
\]

\[
\infer[(Join2)]{
    \Gamma,\tau \vdash H(\bar{y}) \dldeduce Pred, Join \hookrightarrow \phi_1 \land \phi_2
}{
    \Gamma,\tau \vdash Pred \rightsquigarrow \phi_1
    & 
    \Gamma,\tau \vdash H(\bar{y}) \dldeduce Join \hookrightarrow \phi_2
}
\]

\[
\infer[(Sum)]{
    \Gamma,\tau \vdash H(\bar{y}) \dldeduce R(\bar{x}), s=sum~n: R(\bar{z})
        \hookrightarrow s=s'
}{
    s'=\Gamma(H)[\bar{k}].value + n
}
\]
where $\bar{k}$ represents the primary keys of relation $H$, extracted from the
array $\bar{y}$, and $\Gamma(H)[\bar{k}].value$ reads the current sum value.
Note that, unlike the join rules, the literal $R(\bar{x})$ 
here does not join with the aggregation literal, 
because it is only introduced to obtain valid valuations for the rule variables
(every row in table $R$ is a valid valuation).
For each valid valuation, the aggregator computes the aggregate summary 
for the matching rows in table $R$ (Section~\ref{sec:language}).
This applies to all inference rules for aggregators.

\[
\infer[(Max)]{
    \Gamma, \tau \vdash H(\bar{y}) \dldeduce R(\bar{x}), m=max~n: R(\bar{z}) 
        \hookrightarrow \phi
    }
    {
    m' = \Gamma(H)[\bar{k}].value
    & \phi \coloneqq (n > m' \land m=n) \oplus (n \leq m')
    }
\]

\[
\infer[(Min)]{
    \Gamma, \tau \vdash H(\bar{y}) \dldeduce R(\bar{x}), m=min~n: R(\bar{z})
        \hookrightarrow  \phi
    }
    {
    m' = \Gamma(H)[\bar{k}].value
    & 
    \phi \coloneqq (n < m' \land m=n) \oplus (n \geq m')
    }
\]

\[
\infer[(Count)]{
    \Gamma,\tau \vdash H(\bar{y}) \dldeduce R(\bar{x}), c=count: R(\bar{z}) 
        \hookrightarrow \phi
    }{
        \phi \coloneqq c=\Gamma(H)[\bar{k}].value+1
    }
\]

\noindent{\textbf{Encoding individual literals.}}
Following are the inference rules for judgment:
$ \Gamma,\tau \vdash \var{Pred} \rightsquigarrow \phi $,
which encodes individual literals.

\[
\infer[(Lit1)]{
    \Gamma, \tau \vdash R(\bar{x}) \rightsquigarrow \tau = R(\bar{x})
}{
    \tau.rel = R
  }
\quad
\infer[(Lit2)]{
  \Gamma, \tau \vdash R(\bar{x}) \rightsquigarrow \Gamma(R)[\bar{k}] = \bar{v}
}{
    \tau.rel \neq R
}
\]
where $\bar{k}$ represents the primary keys in relational literal $R(\bar{x})$, 
extracted from $\bar{x}$,
and $\bar{v}$ represents the remaining fields in $\bar{x}$.

\[
\infer[(Condition)]{
    \Gamma, \tau \vdash C \rightsquigarrow C
    }{}
\quad
\infer[(Function)]{
    \Gamma, \tau \vdash y = F(\bar{x}) \rightsquigarrow y=F(\bar{x})
    }{}
\]

\noindent{\textbf{Assumptions.}}
\proto assumes that on every new incoming transaction request, 
there is at most one new tuple derived by each rule,
and that there is no recursion in the rules.

Recursion means that there is a mutual dependency between
rules. A rule $r_a$ is dependent to another rule $r_b$
($r_a \rightarrow r_b$)
if and only if $r_b$'s head relation appears in $r_a$'s body,
or there exists another rule $r_c$ such that 
$r_a \rightarrow r_c \land r_c \rightarrow r_b$.

This assumption keeps the size of the transition constraint 
linear to the number of rules in the Decon contract,
thus making the safety verification tractable.
We find this assumption holds for most smart contracts 
in the financial domain, and is true for all of the ten
benchmark contracts in our evaluation.


==> sec_limitation.tex <==
\section{Limitations}

Reason about contract with functions outside of relational logic.

Counter-example generation.

Properties beyond safety.

